CORRECT: Context- and Reference-Augmented Reasoning and Prompting for Fact-Checking

Fact-checking the truthfulness of claims usually requires reasoning over multiple evidence sentences. Oftentimes, evidence sentences may not be always self-contained, and may require additional contexts and references from elsewhere to understand coreferential expressions, acronyms, and the scope of a reported finding. For example, evidence sentences from an academic paper may need contextual sentences in the paper and descriptions in its cited papers to determine the scope of a research discovery. However, most fact-checking models mainly focus on the reasoning within evidence sentences, and ignore the auxiliary contexts and references. To address this problem, we propose a novel method, Context- and Reference-augmented Reasoning and Prompting. For evidence reasoning, we construct a three-layer evidence graph with evidence, context, and reference layers. We design intra- and cross-layer reasoning to integrate three graph layers into a unified evidence embedding. For verdict prediction, we design evidence-conditioned prompt encoder, which produces unique prompt embeddings for each claim. These evidence-conditioned prompt embeddings and claims are unified for fact-checking. Experiments verify the strength of our model.

==> additional_experiments.tex <==
\section{Additional Experiment Results}
\label{sec:additional_experiments}

In the main paper, we mainly show the experiment results with Macro F1 score as evaluation metric. Here we further provide results with Micro F1 scores in Table \ref{table:fully_supervised_micro_f1} and Table \ref{table:5_shot_micro_f1} for fully supervised setting and 5-shot setting, respectively.

Overall, our model predicts veracity more accurately than baselines across all datasets, because of the advantage of incorporating both contextual and referential documents. By comparing to prompting-bases baselines that use natural language prompt, our model achieves better verification accuracy, since continuous and learnable prompt embeddings learned by our proposed evidence-conditioned prompt encoder are flexible and can better adapt to the dataset. Again, MultiVerS is slightly better than our model on SciFact dataset, mainly because most evidence sentences in this dataset are sufficient to verify the claims, and auxiliary referential documents do not bring much additional benefit.

\begin{table*}[t]
	\centering
	\caption{Verdict prediction results on \emph{fully supervised} setting with \emph{Micro F1} score. Results are in percentage.}
	%\vspace{-0.2cm}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{c|cc|cc|cc|cc}
			\toprule
                \multirow{2}{*}{Model} & \multicolumn{2}{c|}{BearFact} & \multicolumn{2}{c|}{Check-COVID} & \multicolumn{2}{c|}{SciFact} & \multicolumn{2}{c}{FEVEROUS-S} \\
			\cline{2-9}
			{} & Gold & Retrieved & Gold & Retrieved & Gold & Retrieved & Gold & Retrieved \\
			\hline
                KGAT & 69.42$ \pm $0.87 & 57.36$ \pm $0.52 & 72.05$ \pm $1.58 & 76.47$ \pm $0.65 & 74.44$ \pm $0.96 & 62.33$ \pm $0.88 & 86.21$ \pm $0.28 & 67.99$ \pm $0.78 \\
                HESM & 63.68$ \pm $1.39 & 58.62$ \pm $0.32 & 63.47$ \pm $0.25 & 71.90$ \pm $1.85 & 72.44$ \pm $0.77 & 53.36$ \pm $2.33 & 83.30$ \pm $0.75 & 68.36$ \pm $0.86 \\
                Transformer-XH & 61.26$ \pm $0.72 & 56.55$ \pm $1.50 & 68.56$ \pm $0.87 & 76.91$ \pm $1.51 & 75.89$ \pm $0.51 & 58.67$ \pm $1.53 & 85.61$ \pm $0.80 & 69.78$ \pm $0.41 \\
                Transformer-XH++ & 64.02$ \pm $1.44 & 58.39$ \pm $1.11 & 70.60$ \pm $0.67 & 78.65$ \pm $0.38 & 77.78$ \pm $0.69 & 60.56$ \pm $1.83 & 85.52$ \pm $0.39 & 70.37$ \pm $0.77 \\
                MultiVerS & 62.93$ \pm $1.17 & 50.69$ \pm $1.46 & 66.65$ \pm $1.71 & 70.70$ \pm $1.73 & 83.68$ \pm $1.40 & \textbf{66.77}$ \pm $\textbf{0.14} & 83.57$ \pm $1.54 & 67.66$ \pm $1.65 \\
                CausalWalk & 69.31$ \pm $1.69 & 60.00$ \pm $0.69 & 71.86$ \pm $1.54 & 71.68$ \pm $2.48 & 77.34$ \pm $2.30 & 59.00$ \pm $1.20 & 86.42$ \pm $0.92 & 71.51$ \pm $1.66 \\
                \hline
                GPT2-PPL & 40.00$ \pm $2.43 & 39.49$ \pm $0.73 & 32.75$ \pm $0.62 & 32.54$ \pm $0.93 & 31.50$ \pm $0.71 & 31.24$ \pm $1.56 & 54.33$ \pm $0.06 & 54.23$ \pm $0.01 \\
                ProToCo & 56.03$ \pm $0.24 & 35.57$ \pm $2.35 & 37.12$ \pm $1.10 & 32.75$ \pm $2.31 & 60.00$ \pm $1.53 & 31.17$ \pm $0.71 & 54.21$ \pm $0.67 & 44.71$ \pm $1.95 \\
                ProgramFC & 62.00$ \pm $2.83 & 54.63$ \pm $3.66 & 65.50$ \pm $2.12 & 72.36$ \pm $1.85 & 65.40$ \pm $3.78 & 59.76$ \pm $3.54 & 86.48$ \pm $0.33 & 69.50$ \pm $2.12 \\
                \hline
                P-Tuning v2 & 70.69$ \pm $0.49 & 60.34$ \pm $0.15 & 72.93$ \pm $1.85 & 77.32$ \pm $1.96 & 80.34$ \pm $0.94 & 57.44$ \pm $1.83 & 87.16$ \pm $0.33 & 70.56$ \pm $0.54 \\
                \hline
                JustiLM & 62.41$ \pm $1.25 & 48.49$ \pm $2.21 & 59.71$ \pm $2.56 & 61.71$ \pm $2.05 & 72.20$ \pm $1.85 & 54.74$ \pm $0.82 & 81.60$ \pm $0.33 & 68.38$ \pm $1.45 \\
                \hline
                CORRECT & \textbf{74.60}$ \pm $\textbf{1.11} & \textbf{61.84}$ \pm $\textbf{0.11} & \textbf{75.33}$ \pm $\textbf{0.93} & \textbf{80.83}$ \pm $\textbf{0.76} & \textbf{85.17}$ \pm $\textbf{0.71} & 63.50$ \pm $1.17 & \textbf{88.51}$ \pm $\textbf{0.19} & \textbf{75.35}$ \pm $\textbf{0.28} \\
			\bottomrule
		\end{tabular}
	}
	%\vspace{-0.3cm}
	\label{table:fully_supervised_micro_f1}
\end{table*}

\begin{table*}[t]
	\centering
	\caption{Verdict prediction results on \emph{5-shot} setting with \emph{Micro F1} score. Results are in percentage.}
	%\vspace{-0.2cm}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{c|cc|cc|cc|cc}
			\toprule
                \multirow{2}{*}{Model} & \multicolumn{2}{c|}{BearFact} & \multicolumn{2}{c|}{Check-COVID} & \multicolumn{2}{c|}{SciFact} & \multicolumn{2}{c}{FEVEROUS-S} \\
			\cline{2-9}
			{} & Gold & Retrieved & Gold & Retrieved & Gold & Retrieved & Gold & Retrieved \\
			\hline
                KGAT & 44.66$ \pm $0.25 & 36.78$ \pm $3.86 & 37.55$ \pm $2.86 & 50.98$ \pm $1.13 & 42.22$ \pm $3.06 & 36.78$ \pm $3.52 & 51.13$ \pm $1.55 & 51.66$ \pm $1.38 \\
                HESM & 48.85$ \pm $2.42 & 28.97$ \pm $3.26 & 36.68$ \pm $5.15 & 50.11$ \pm $3.22 & 39.56$ \pm $2.45 & 35.89$ \pm $4.67 & 56.33$ \pm $0.91 & 53.68$ \pm $0.37 \\
                Transformer-XH & 32.53$ \pm $3.13 & 40.80$ \pm $3.32 & 41.67$ \pm $2.19 & 51.63$ \pm $1.16 & 48.89$ \pm $2.84 & 35.11$ \pm $1.95 & 52.94$ \pm $2.65 & 51.56$ \pm $0.73 \\
                Transformer-XH++ & 37.93$ \pm $4.10 & 35.06$ \pm $3.66 & 41.40$ \pm $1.78 & 52.41$ \pm $1.22 & 50.00$ \pm $0.85 & 36.67$ \pm $1.65 & 59.97$ \pm $1.50 & 53.23$ \pm $1.19 \\
                MultiVerS & 40.86$ \pm $0.74 & 39.49$ \pm $1.70 & 41.01$ \pm $1.29 & 49.82$ \pm $1.56 & \textbf{54.99}$ \pm $\textbf{1.90} & 43.33$ \pm $1.74 & 51.39$ \pm $1.33 & 51.84$ \pm $1.54 \\
                CausalWalk & 45.52$ \pm $3.47 & 41.38$ \pm $3.24 & 37.70$ \pm $4.59 & 43.79$ \pm $3.25 & 44.02$ \pm $2.70 & 41.78$ \pm $2.71 & 60.60$ \pm $1.98 & 55.20$ \pm $4.18 \\
                \hline
                GPT2-PPL & 36.38$ \pm $4.14 & 40.69$ \pm $0.49 & 33.19$ \pm $0.67 & 34.62$ \pm $0.72 & 29.44$ \pm $2.50 & 29.00$ \pm $1.46 & 53.02$ \pm $1.11 & 53.11$ \pm $1.12 \\
                ProToCo & 51.03$ \pm $2.44 & 33.80$ \pm $2.44 & 41.05$ \pm $2.47 & 34.50$ \pm $2.31 & 51.55$ \pm $2.27 & 36.78$ \pm $1.35 & 54.72$ \pm $1.32 & 42.45$ \pm $2.73 \\
                ProgramFC & 38.45$ \pm $2.19 & 38.28$ \pm $0.49 & 37.55$ \pm $0.38 & 50.00$ \pm $1.08 & 49.93$ \pm $0.36 & 36.17$ \pm $1.25 & 52.94$ \pm $2.67 & 51.94$ \pm $0.25 \\
                \hline
                P-Tuning v2 & 48.70$ \pm $1.95 & 41.90$ \pm $3.10 & 41.05$ \pm $3.88 & 52.07$ \pm $3.09 & 45.78$ \pm $1.07 & 37.67$ \pm $1.85 & 58.02$ \pm $1.68 & 52.06$ \pm $0.76 \\
                \hline
                JustiLM & 42.70$ \pm $1.64 & 37.72$ \pm $5.08 & 40.82$ \pm $2.20 & 46.73$ \pm $1.53 & 47.41$ \pm $1.07 & 33.00$ \pm $1.58 & 52.54$ \pm $1.71 & 49.38$ \pm $1.60 \\
                \hline
                CORRECT & \textbf{51.72}$ \pm $\textbf{1.04} & \textbf{42.76}$ \pm $\textbf{0.73} & \textbf{43.37}$ \pm $\textbf{1.82} & \textbf{54.46}$ \pm $\textbf{0.76} & 53.00$ \pm $1.30 & \textbf{44.36}$ \pm $\textbf{0.84} & \textbf{63.33}$ \pm $\textbf{0.91} & \textbf{57.14}$ \pm $\textbf{0.82} \\
			\bottomrule
		\end{tabular}
	}
	%\vspace{-0.3cm}
	\label{table:5_shot_micro_f1}
\end{table*}

==> notations.tex <==
\section{Mathematical Notations}
\label{sec:notations}

Here we provide a summary of main mathematical notations used in the main paper in Table \ref{table:notation_table}.

\begin{table*}[t]
	\centering
	\caption{Summary of mathematical notations.}
	%\vspace{-0.3cm}
	%\resizebox{\columnwidth}{!}{
		\begin{tabular}{c|l}
			\toprule
			Notation  & Description  \\
			\hline
			$ \mathcal{D} $ & a fact-checking dataset \\
			$ \mathcal{X} $ & a set of $ N=|\mathcal{X}| $ claims \\
			$ \mathcal{E} $ & a corpus of evidence sentences \\
			$ \mathcal{C} $ & a set of contextual documents \\
                $ \mathcal{R} $ & a set of referential documents \\
			$ \mathcal{N}_{\text{ref}}(e) $ & evidence sentence $ e $'s referential documents \\
                $ \mathcal{N}_{\text{evid}}(x) $ & claim $ x $'s retrieved evidence sentences \\
                $ \mathcal{Y} $ & a set of labels \\
                $ \textbf{h}_{e,\text{CLS}}^{(l)} $ & evidence sentence $ e $'s [CLS] token embedding at the $ l $-th step \\
                $ \hat{\textbf{h}}_{e}^{(l)} $ & evidence sentence $ e $'s embedding after intra-layer reasoning \\
                $ \hat{\textbf{h}}_{c}^{(l)} $ & aggregated contextual document embedding \\
                $ \hat{\textbf{h}}_{r}^{(l)} $ & aggregated referential document embedding \\
                $ \widehat{\textbf{H}}_{e}^{(l)} $ & evidence sentence $ e $'s augmented embedding matrix \\
                $ \bm{\pi}_{m,y} $ & the $ m $-th prompt embedding for class $ y $ \\
                $ \textbf{h}_{m,y} $ & the $ m $-th base prompt embedding for class $ y $ \\
			\bottomrule
		\end{tabular}
	%}
	%\vspace{-0.5cm}
	\label{table:notation_table}
\end{table*}

==> original_template.tex <==
\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl\_latex.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
  \centering
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\"a}|     & {\"a}           \\
    \verb|{\^e}|     & {\^e}           \\
    \verb|{\`i}|     & {\`i}           \\
    \verb|{\.I}|     & {\.I}           \\
    \verb|{\o}|      & {\o}            \\
    \verb|{\'u}|     & {\'u}           \\
    \verb|{\aa}|     & {\aa}           \\\hline
  \end{tabular}
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\c c}|    & {\c c}          \\
    \verb|{\u g}|    & {\u g}          \\
    \verb|{\l}|      & {\l}            \\
    \verb|{\~n}|     & {\~n}           \\
    \verb|{\H o}|    & {\H o}          \\
    \verb|{\v r}|    & {\v r}          \\
    \verb|{\ss}|     & {\ss}           \\
    \hline
  \end{tabular}
  \caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
  \label{tab:accents}
\end{table}

As much as possible, fonts in figures should conform
to the document fonts. See Figure~\ref{fig:experiments} for an example of a figure and its caption.

Using the \verb|graphicx| package graphics files can be included within figure
environment at an appropriate point within the text.
The \verb|graphicx| package supports various optional arguments to control the
appearance of the figure.
You must include it explicitly in the \LaTeX{} preamble (after the
\verb|\documentclass| declaration and before \verb|\begin{document}|) using
\verb|\usepackage{graphicx}|.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{example-image-golden}
  \caption{A figure with a caption that runs for more than one line.
    Example image is usually available through the \texttt{mwe} package
    without even mentioning it in the preamble.}
  \label{fig:experiments}
\end{figure}

\begin{figure*}[t]
  \includegraphics[width=0.48\linewidth]{example-image-a} \hfill
  \includegraphics[width=0.48\linewidth]{example-image-b}
  \caption {A minimal working example to demonstrate how to place
    two images side-by-side.}
\end{figure*}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation:
\begin{quote}
\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
  \centering
  \begin{tabular}{lll}
    \hline
    \textbf{Output}           & \textbf{natbib command} & \textbf{ACL only command} \\
    \hline
    \citep{Gusfield:97}       & \verb|\citep|           &                           \\
    \citealp{Gusfield:97}     & \verb|\citealp|         &                           \\
    \citet{Gusfield:97}       & \verb|\citet|           &                           \\
    \citeyearpar{Gusfield:97} & \verb|\citeyearpar|     &                           \\
    \citeposs{Gusfield:97}    &                         & \verb|\citeposs|          \\
    \hline
  \end{tabular}
  \caption{\label{citation-guide}
    Citation commands supported by the style file.
    The style is based on the natbib package and supports all natbib citation commands.
    It also supports commands defined in previous ACL style files for compatibility.
  }
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

A possessive citation can be made with the command \verb|\citeposs|.
This is not a standard natbib command, so it is generally not compatible
with other style files.

\subsection{References}

\nocite{Ando2005,andrew2007scalable,rasooli-tetrault-2015}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Equations}

An example equation is shown below:
\begin{equation}
  \label{eq:example}
  A = \pi r^2
\end{equation}

Labels for equation numbers, sections, subsections, figures and tables
are all defined with the \verb|\label{label}| command and cross references
to them are made with the \verb|\ref{label}| command.

This an example cross-reference to Equation~\ref{eq:example}.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgments}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya,
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu,
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan,
NAACL 2017 by Margaret Mitchell,
ACL 2012 by Maggie Li and Michael White,
ACL 2010 by Jing-Shin Chang and Philipp Koehn,
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui,
ACL 2005 by Hwee Tou Ng and Kemal Oflazer,
ACL 2002 by Eugene Charniak and Dekang Lin,
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

% Bibliography entries for the entire Anthology, followed by custom entries
%\bibliography{anthology,custom}
% Custom bibliography entries only
\bibliography{custom}

\appendix

\section{Example Appendix}
\label{sec:appendix}

This is an appendix.
